Exposing Computer Generated Images by Using Deep Convolutional Neural Networks

The recent computer graphics developments have upraised the quality of the generated digital content, astonishing the most skeptical viewer. Games and movies have taken advantage of this fact but, at the same time, these advances have brought serious negative impacts like the ones yielded by fakeimages produced with malicious intents. Digital artists can compose artificial images capable of deceiving the great majority of people, turning this into a very dangerous weapon in a timespan currently know as Fake News/Post-Truth" Era. In this work, we propose a new approach for dealing with the problem of detecting computer generated images, through the application of deep convolutional networks and transfer learning techniques. We start from Residual Networks and develop different models adapted to the binary problem of identifying if an image was or not computer generated. Differently from the current state-of-the-art approaches, we don't rely on hand-crafted features, but provide to the model the raw pixel information, achieving the same 0.97 of state-of-the-art methods with two main advantages: our methods show more stable results (depicted by lower variance) and eliminate the laborious and manual step of specialized features extraction and selection.

==> 03_proposed_method.tex <==
\section{Proposed Method}
\label{sec:proposedmethod}

\AT{The CG detection method proposed in this work relies upon a deep CNN architecture to classify each image from the dataset using the raw RGB pixels values as features, without the need for manual feature extraction. The deep CNN deployed is based on the ResNet-50 model~\cite{he2016deep} and the method uses transfer learning techniques~\cite{yosinski2014transferable}. Before presenting the details of the model and its architecture, these fundamental concepts will be introduced.}

\subsection{ResNet-50}

\AT{Residual Networks (ResNet)~\cite{he2016deep} can be classified as convolutional neural networks (CNN). These CNNs, in turn, can be defined as neural networks that have at least one layer using the convolution operation~\cite{Goodfellow-et-al-2016}. Mathematically speaking, the convolution operation can be view as a weighted average operation of two functions ($x$ and $w$), where one of them ($w$) is a probability density function. More formally:}

\AT{$$ s(t) = (x * w)(t) = \int x(a) w(t-a) da $$}

\AT{In practice, due to the commutative property, the convolution operation is usually implemented as the cross-correlation function~\cite{Goodfellow-et-al-2016}. For example, assuming the function $x$ as a two-dimensional input image $I$ and the probability density function $w$ as a function $K$ (usually called \textit{kernel} in machine learning terminology), the function $S$ below is the convolution of \textit{kernel} $K$ over the image $I$:}

\AT{$$ S(i,j) = (I * K)(i,j) = \sum_{m} \sum_{n} I(i+m,j+n)K(m,n) $$}

\AT{In machine learning nomenclature, the function $S$ is usually called a \textit{feature map}. Among many interesting properties that convolutions convey, one of paramount importance is the robustness to translation in the recognition of patterns. If a kernel $K$ is specialized in recognizing circles, the convolution of this kernel over the image will identify circles no matter where they occur in the image.}

\AT{Besides convolutions, CNNs usually have some non-linear activation functions (like sigmoid or rectified linear functions) and pooling layers that have the effect of turning the representation invariant to small translations in the image~\cite{Goodfellow-et-al-2016}.}

\AT{Residual Networks (ResNets)~\cite{he2016deep} are deep convolutional networks where the basic idea is to skip blocks of convolutional layers by using shortcut connections to form conceptual shortcut blocks named residual blocks. The residual block can be formally described in the general form:}

\AT{$$ \mathcal{Y}_{l}(\mathbf{x},W) = f(h(\mathbf{x}) + \mathcal{F}(\mathbf{x},W))$$}

\AT{where $\mathbf{x}$ is the input of the block, $h$ is the \textit{shortcut} function (crucial to ResNet and better explained below), $\mathcal{F}$ is the mapping done by a block of one or more consecutive convolutional layers (being skipped), $W$ is the weights of these convolutional layers, $f$ is a rectified linear unit (ReLU) and $\mathcal{Y}_{l}$ is the mapping that describes the residual block $l$ as a function of the input $\mathbf{x}$ and the weights $W$. The shortcut function is usually the identity function (or a very simple convolutional layer when a dimensional compatibility is needed) and its purpose is to speed the learning of the mapping $\mathcal{F}$ as a perturbation of the input $\mathbf{x}$, starting this learning from a point near the identity function. This is faster to learn than from a random point near the zero-mapping (as done by previous architectures) and is one of the key contributions of Residual Networks.}

%In ResNet-50 architecture, the basic blocks, also called bottleneck blocks, are composed of a sequence of convolutional layers with filters of size $1\times1$, $3\times3$ and $1\times1$ respectively, that follow two simple design rules: (i) for the same output feature map size, the layers have the same number of filters; and (ii) if the feature map size is halved, the number of filters is doubled. The down-sampling is performed directly by convolutional layers that have a stride of 2 and batch normalization \cite{ioffe2015batch} is performed right after each convolution and before ReLU activation. Figure~\ref{fig:bottleneckblocks} tries to clarify this set-up.

\AT{In ResNet-50 architecture, the basic residual blocks, also called bottleneck blocks, are composed of a sequence of three convolutional layers with filters of size $1\times1$, $3\times3$ and $1\times1$ respectively. The down-sampling is performed directly by convolutional layers that have a stride of 2 and batch normalization \cite{ioffe2015batch} is performed right after each convolution and before ReLU activation.}

%The identity shortcuts can be directly used when the input and output are of the same dimensions. When the dimensions increase, two options are considered: (i) The shortcut still performs identity mapping, with extra zero entries padded for increasing dimensions. This option introduces no extra parameter; (ii) The projection shortcut is used to match dimensions (done by $1\times1$ convolutions). For both options, when the shortcuts go across feature maps of two sizes, they are performed with a stride of 2.

\AT{The identity shortcuts can be directly used when the input and output feature maps are of the same dimensions. When the dimensions change, two options are considered: (i) The shortcut still performs identity mapping, with extra zero entries padded for increasing filter dimensions (depth). This option introduces no extra parameter; (ii) A $1\times1$ convolution layer is used to match the dimensions. This is called  \textit{projection} shortcut. For both options, when the shortcuts go across feature maps of two sizes, they are performed with a stride of 2. Figure~\ref{fig:bottleneckblocks} tries to clarify this set-up.}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.99\textwidth]{images/bottleneckblocks2.pdf}
  \caption{Bottleneck Blocks for ResNet-50 (left: identity shortcut; right: projection shortcut).}
 \label{fig:bottleneckblocks}
\end{figure*}

The network ends with a global average pooling layer and a 1000-way fully-connected layer with softmax activation. The total number of weighted layers is 50.

\subsection{Transfer Learning}
\label{sec:transferlearning}

\TJ{Deep learning techniques usually require a very large number of samples and demands a heavy computing effort. In this scenario, transfer learning ~\cite{yosinski2014transferable} has gained a lot of attention. It represents the possibility to transfer the knowledge learned from one problem to another problem. For neural networks, the transfer learning process consists, in practice, in transferring the parameters of a (source) neural network that was previously trained for a particular dataset for a specific task to another (target) network with a different dataset to solve a different problem.}

\TJ{A typical transfer learning procedure implies in using an already trained base network and copying all the parameters from the first $n$ layers to the first $n$ layers of the target network. Then, a supervised training is performed only on the remaining layers that were not copied. Since the task is different and probably so is  number of classes, the last layer has to be modified to contain the same amount of neuron as the number of classes or it can be replaced by another classifier.
During this training, the copied layers can be left fixed, or it can fine-tuned by allowing the backpropagation process into the copies parameters. Usually fine-tuning  improves the accuracy, however, when the number of parameters is big and the numbers of samples is small, this may result in overfitting and fine-tuning should not be used. }

\TJ{In traditional supervised learning, the common sense was settled that the training should always be performed specifically for a given task and dataset and the transfer learning approach could sound senseless. However, in general, deep neural networks present a particular characteristic which is to learn features in the first layers that are more general and not specific to that particular dataset and problem. That makes that knowledge reusable for other problems and dataset. On the other hand, the knowledge learned on the last layers of the neural network are more specific for that task.}

\TJ{Transfer learning is very handy because it avoids the  task of training the network. Since the architecture is very deep, training it represents an enormous computational efforts requiring expensive high processing computers, usually using multiple high-end GPU units. Another problem in training deep networks from scratch is that it required a vary large number of samples, otherwise is will overfit the data. Transfer learning significantly mitigates this two problems, enabling the use of deep learning even when the target dataset is small or when there is limited computing resources. Recent studies have taken advantage of this fact to obtain state-of-the-art results~\cite{donahue2014decaf}\cite{zeiler2014visualizing}\cite{sermanet2013overfeat}, which evidences the generality of the features learned in the first layers of the network.}

\TJ{In this work, we apply transfer learning technique by using the same parameters of the ResNet-50 network trained for the ImageNet 2012 competition~\cite{russakovsky2015imagenet} which provided a 1.28 million images dataset from 1000 classes. The first 49 layers of the network were copied to a new ResNet-50 network and we removed the last layer, replacing it by another classifier. We have not used fine-tuning during the training due to the relatively small dataset.}


\subsection{Top Classifier}
\label{sec:classifiers}

In the proposed method, the last layer of the ResNet-50 is replaced by another classifier and we have evaluated four different classifier for this task.

\subsubsection{Softmax}

The softmax function is a generalization of the binary logistic regression to multiple classes. 


\subsubsection{KNN}

\subsubsection{XGBoost}

\subsubsection{SVM}



\subsection{Complete Model Architecture}

\AT{
Our proposed deep CNN model uses transfer learning techniques, leveraging the outcomes of residual learning presented by the ResNet-50. The final model architecture, with its pipeline depicted in Figure \ref{fig:overview}, consists of:
}

\begin{enumerate}
    \item an initial pre-processing stage;
    \item a sequence of many convolutional layers based on the first 49 layers of ResNet-50 and;
    \item a top classifier replacing the original 1000 fully-connected softmax layer.
\end{enumerate}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.99\textwidth]{images/overview.pdf}
  \caption{Overview of proposed method. Transferring ResNet-50 parameters to our model to extract bottleneck features, which are used to train different classifiers.}
 \label{fig:overview}
\end{figure*}

\AT{
The dataset used consists of variable-resolution images while our model requires a constant input dimensionality. Therefore, we resize the images to a fixed resolution of $224\times224$ and, for each pixel, we subtract the mean RGB value computed over the ImageNet dataset (as proposed by \citeauthor{krizhevsky2012imagenet}~\cite{krizhevsky2012imagenet}). These two operations are performed by the pre-processing layer.
}

\AT{
After pre-processing the dataset images, we apply the transfer learning techniques explained in Section \ref{sec:transferlearning}. In our CNN model, after the pre-processing, we use the first 49 layers of ResNet-50 with their weights trained on ImageNet as a features extractor (red box named ``Bottleneck Features Extractor'' of Figure \ref{fig:overview}) to generate a set of features with the correspondent label associated. These labelled features, also called bottleneck features\footnote{Bottleneck term refers to a neural network topology where the hidden layer has significantly lower dimensionality than the input layer, assuming that such layer --- referred to as the bottleneck --- compresses the information needed for mapping the neural network input to the neural network output, increasing the system robustness to noise and overfitting. Conventionally, bottleneck features are the output generated by the bottleneck layer.} are the activation maps generated by the average pooling layer (the 49\textsuperscript{th} layer of ResNet-50), ignoring the last 1000 fully-connected softmax layer.
}

\AT{
These bottleneck features are used to train a top classifier that will make the final prediction of CG images. This classifier has the same role as the original softmax layer at the end of ResNet-50, adapting the network to the binary problem of CG image detection. The replacement of this softmax layer, with thousands of parameters, associated with the transfer learning techniques used (no learning happens at the convolutional layers), allowed us to deploy a very deep CNN for the CG image detection problem without the requirement of millions of CG/PG labelled images, besides significantly reducing the training time. 
}

\AT{
Once finished the training process, our final deep CNN model used for testing is made up of the pre-processing layer, the Bottleneck Features Extractor and a top classifier (network on the right of Figure \ref{fig:overview}). Lots of different classifiers were trained as top classifiers to discover which one performs best for the task of CG image detection. Section \ref{sec:classifiers} will delve into the details of each type used.
}


